Mapping of Sparse 3D Data using Alternating Projection

We propose a novel technique to register sparse 3D scans in the absence of texture. While existing methods such as KinectFusion or Iterative Closest Points (ICP) heavily rely on dense point clouds, this task is particularly challenging under sparse conditions without RGB data. Sparse texture-less data does not come with high-quality boundary signal, and this prohibits the use of correspondences from corners, junctions, or boundary lines. Moreover, in the case of sparse data, it is incorrect to assume that the same point will be captured in two consecutive scans. We take a different approach and first re-parameterize the point-cloud using a large number of line segments. In this re-parameterized data, there exists a large number of line intersection (and not correspondence) constraints that allow us to solve the registration task. We propose the use of a two-step alternating projection algorithm by formulating the registration as the simultaneous satisfaction of intersection and rigidity constraints. The proposed approach outperforms other top-scoring algorithms on both Kinect and LiDAR datasets. In Kinect, we can use 100X downsampled sparse data and still outperform competing methods operating on full-resolution data.

==> files/exp.tex <==
\section{Experiments}

We used two datasets for evaluation. 

\noindent
{\bf TUM Dataset}~\cite{sturm12} consists of sequences of Kinect RGBD data captured in an indoor environment. The sensor resolution is 640x480, at 30 fps. The sequences come with a ground truth trajectory of the sensor, obtained from a high-accuracy motion-capture system. Our algorithms only use the depth information from this dataset, downsampled by a factor of 100. In the results shown in the paper, previous methods use the full point-cloud. 

\noindent
{\bf KITTI Dataset}~\cite{Geiger2012CVPR} consists of LiDAR point-clouds collected from the top of a moving vehicle. The LiDAR sensor captures roughly 10 fps (frames per second), with about 100k points per frame. 

We used two evaluation metrics:

\noindent
\textbf{Relative Pose Error (RPE):} As proposed in \cite{sturm12}, we compute the error in the relative pose between successive frames, and report the translation error in meters and rotation error in degrees respectively.

\vspace{.25cm}
\noindent
\textbf{Translation and Rotation Error along the trajectory:} This metric is used in \cite{Geiger2012CVPR} and on their online leaderboard. For all sub-sequences of length 100m, 200m, $\ldots$, 800m, we compute the translation and rotation errors per unit length of the trajectory. Translation error is reported as a percentage value, and rotation error in degrees per meter.

% \subsection{RANSAC Metrics}
% For the ransac distance metric we use....

% We apply RANSAC to detect planes for the 3L1P and 1L2P methods. On KITTI dataset, we apply 200 trials on each frame and accept one plane if it has more than 500 inlier points, which are with 8 cm from the plane.  
%\subsection{Synthetic Evaluation}
%In this subsection we show some experimental results to evaluate the efficiency and robustness of the minimal solver proposed in Sec.~\ref{sec:mix}. For this purpose, we consider synthetic data. We randomly generated 3D straight lines ans 3D planes with in a 10 square meter box. These data is generated by: 1) for lines considering two lines edge points; and 2) 3D planes defined by the 3D points. To these 3D points, we inject random noise with mean zero and standard deviation with variable {\tt Noise STD}. A total of 100 3D line intersection and 100 3D plane correspondences were randomly generated for each trial.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.23\textwidth]{figs/rotation_numerical.jpg} \hfill
%     \includegraphics[width=0.23\textwidth]{figs/translation_numerical.jpg}
%     \caption{Numerical experiments for the two efficient minimal solvers proposed in this paper (combination of line intersection and plane correspondences).}
%     \label{fig:numerical}
% \end{figure}

%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=0.235\textwidth]{figs/rotation_noise.jpg}
%    \hfill
%    \includegraphics[width=0.225\textwidth]{figs/translation_noise.jpg}
%    \caption{Noise experiments for the two minimal solvers proposed in this paper. We use all the three solvers proposed in this paper within the RANSAC framework.}
%    \label{fig:noise}
%\end{figure}

%We start by testing the robustness of the proposed solvers. For that purpose, we consider the trials with noise variable {\tt Noise STD} applied to the 3D points that define both the lines and the planes ranging from $1$ to $10[cm]$. For each value of the noise, we randomly generate $100$ trials, and for each of the trials we run the proposed solvers: 1) the seven line intersection; 2) the three line intersection and one plane correspondence; and 3) the one line intersection and two plane correspondences, within the RANSAC framework~\cite{fischler81}. For the RANSAC distance, we use only the 3D line intersection distances presented in the previous subsection. We use $100$ RANSAC cycles, and a minimum of $50\%$ of inliers for a pose to be considered as valid. The results for both solvers are shown in Fig.~\ref{fig:noise}. As we can see from these results, the results are similar. The case of three 3D lines and one 3D plane perform slightly worse than the others.

